OnlineAnySeg: Online Zero-Shot 3D Segmentation by Visual Foundation Model Guided 2D Mask Merging

Online zero-shot 3D instance segmentation of a progressively reconstructed scene is both a critical and challenging task for embodied applications. With the success of visual foundation models (VFMs) in the image domain, leveraging 2D priors to address 3D online segmentation has become a prominent research focus. Since segmentation results provided by 2D priors often require spatial consistency to be lifted into final 3D segmentation, an efficient method for identifying spatial overlap among 2D masks is essential - yet existing methods rarely achieve this in real time, mainly limiting its use to offline approaches. To address this, we propose an efficient method that lifts 2D masks generated by VFMs into a unified 3D instance using a hashing technique. By employing voxel hashing for efficient 3D scene querying, our approach reduces the time complexity of costly spatial overlap queries from $O(n^2)$ to $O(n)$. Accurate spatial associations further enable 3D merging of 2D masks through simple similarity-based filtering in a zero-shot manner, making our approach more robust to incomplete and noisy data. Evaluated on the ScanNet and SceneNN benchmarks, our approach achieves state-of-the-art performance in online, zero-shot 3D instance segmentation with leading efficiency.

==> fig/fig_ablation_criteria.tex <==
\begin{figure}[ht]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.75\linewidth, trim=0 0 0 0, clip]{fig/pdf/Ablation_criteria.pdf}

   \caption{\textbf{Segmentation accuracy using only partial of merging criteria.}}
   \label{fig:ablation_criteria}
\end{figure}

==> fig/fig_rebuttal_speed_comp.tex <==
\begin{figure}[h!]
  \centering
   \includegraphics[width=0.9\linewidth]{fig/pdf/rebuttal_speed_comp.pdf}
   \label{fig:rebuttal_speed}
\end{figure}

==> sec/3_method_bkp.tex <==
\section{Method}
\label{sec:method}

\input{fig/fig_pipeline}


%-------------------------------------------------------------------------
Given a stream of posed RGB-D frames $\{x_t=(C_t, D_t, T_t) | t=0, 1, ..., T\}$, where $C_t \in \mathbb{R}^{H \times W \times 3}$, $D_t \in \mathbb{R}^{H \times W}$ and $T_t \in \mathbb{R}^{4 \times 4}$ denote color image, depth image and camera pose respectively. Our goal is to segment all instances of the reconstructed 3D scene in an online manner. The output of our method includes the point cloud of reconstructed scene $S$, a set of 3D instance masks over $S$, and their corresponding open-vocabulary semantic features. 

% Notably, unlike many existing offline Open-Vocabulary segmentation methods, our approach is designed specifically for online tasks. That is, at any timestamp $t$, our method can only access and utilize data from time $0$ to $t-1$, while also processing incoming frame $x_t$ in real-time.\jiazhao{This is repeated, add this description in previous paragrph}


%-------------------------------------------------------------------------
\subsection{Overview}
\label{subsec:overview}
The overall pipeline of our method is illustrated in \cref{fig:pipeline}, which outlines the flow and key modules of our zero-shot online segmentation process. We employ a hashed voxel volume, denoted as $\mathit{Vol}$, for scene representation and maintain a Global Mask Database $G$ to store extracted information of detected masks with spatial association. Each input frame is processed sequentially: first, it is integrated into $\mathit{Vol}$, and then its color image $C_t$ is fed to a pre-trained Visual Foundation Model (VFM) to generate 2D masks. Each detected 2D mask is subsequently lifted to a 3D mask through back-projection, and the corresponding hit voxels are extracted and inserted into the hash table (\cref{subsec:mask_scene_rep}) to label the overlap associations. In parallel, relevant information of each mask is extracted and stored(\cref{subsec:mask_info_extract}).

As more 2D masks are detected from newly scanned frames, merging periodically the 2D masks belonging to the same 3D instance is necessary. The mask merging process is guided by their ioverlap associations and feature similarity (\cref{subsec:online_mask_merging}). At the end of the input sequence, we can extract the reconstructed scene from the global volume, and each 3D instance's corresponding point cloud can also be accessed from the continuously updated hash table.


%-------------------------------------------------------------------------
\subsection{Mask-Scene Representation}
\label{subsec:mask_scene_rep}
% \input{fig/fig_scenerep}
\paragraph{Mask-Scene Association}
For an incoming frame $x_t=(C_t, D_t, T_t)$, we adopt CropFormer~\cite{qi2022high} to generate entity-level 2D masks in $C_t$. Each detected mask is then lifted into 3D space using the depth image $D_t$, frame pose $P_t$, and camera intrinsics. The resulting back-projected point cloud is voxelized to a set of voxels.

Unlike many existing offline segmentation methods~\cite{yan2024maskclustering, lu2023ovir, schult2022mask3d, takmaz2023openmask3d, yin2024sai3d, nguyen2024open3dis}, which take the scene point cloud as input and operate on it, online segmentation tasks require simultaneous scene reconstruction. We adopt a hashed voxel volume~\cite{newcombe2011kinectfusion, izadi2011kinectfusion, dong2022ash, yamazaki2024open} as our scene representation, with voxels organized in an add-only hash table $H$.

In addition to the TSDF value, each hash entry for a voxel $v_k$ maintains a list of masks that include $v_k$. When a new mask is detected, its ID is appended to the lists of all corresponding voxels.
% An illustration of our scene representation can be found in \cref{fig:scenerep}.


\paragraph{Global Mask Database}
For all $n_t$ masks detected up to timestamp $t$, we maintain a Global Mask Database $G_t$ to store their key information, which is updated accordingly as masks are added or merged (\cref{subsec:online_mask_merging}). Specifically, $M_t=\{ V_t, H_t, F^G_t, F^S_t, W_t, I_t \}$, where $V_t$ records each mask's voxel set, and $H_t$ is the hash table at this timestamp.n

The semantic and geometric feature matrices, $F^S_t \in \mathbb{R}^{n_t \times d_s}$ and $F^M_t \in \mathbb{R}^{n_t \times d_g}$, store the semantic and geometric features of all masks, with $d_s$ and $d_g$ indicating the dimensionalities of the semantic and geometric features respectively.

Each detected mask is initially assigned a weight of 1. When masks are merged, their weights are summed to determine the weight of the new mask. The weight of each mask is stored in the diagonal matrix $W_t=\operatorname{diag}(w_1, w_2, \dots, w_{n_t})$, where $w_i$ represents the weight of the $i$-th mask.

Additionally, $I_t$ records the \textbf{inclusion ratio} of each pair of masks (introduced in \cref{subsec:mask_info_extract}), which indicates the spatial associations between masks and plays a significant role in the mask merging stage (\cref{subsec:online_mask_merging}). The value at position $[a,b]$ in $I_t$ represents the inclusion ratio of the $a$-th mask to the $b$-th mask.


%-------------------------------------------------------------------------
\subsection{Mask-Mask Information Extraction}
\label{subsec:mask_info_extract}
To fuse all masks detected across different frames into 3D instances, the core of our online segmentation method involves dynamically recording and adjusting the associations between all masks, including their spatial overlap, semantic feature similarity and geometric feature similarity, which serve as different criteria for mask merging, as detailed in \cref{subsec:online_mask_merging}. In the following paragraphs, we first introduce inclusion ratio, which describe the degree of overlap between a pair of masks. Then, we introduce the extraction of both semantic feature and geometric feature for a mask.

\paragraph{Inclusion Ratio}
The key to evaluating the spatial associations between two masks lies in their degree of overlap. To quantify this, we propose to leverage the \textbf{inclusion ratio}, as defined below, which can be computed online based on our voxel hashing-based scene representation.

Given any two masks in the Global Mask Database, denoted as $m_a$ and $m_b$, with their corresponding voxel sets $V_a$ and $V_b$, and frame sets $X(m_a)$ and $X(m_b)$, our primary concern is the proportion of $m_a$ that includes $m_b$ (and vice versa). To compute it, first we need to identify the part of $m_b$ that is visible to $m_a$. This can be done by projecting all voxels in $V_b$ into the frame set of $m_a$. The visible voxels are denoted as $\mathit{Vis}(V_b, X(m_a))=\{v_i \in V_b | v_i \rightarrow X(m_a) \}$. We can then compute their overlap by querying the hash table $H_t$ with $V_a$, yielding the intersection $V_a \cap V_b$. With this, the \textbf{inclusion ratio} of $m_a$ to $m_b$ is defined as follows:
\begin{equation}
    \mathit{ir}_{(a,b)}=\frac{V_a \cap V_b}{\mathit{Vis}(V_b, X(m_a))}
    \label{eq:IR}
\end{equation}
This value measures the extent to which $m_a$ and $m_b$ share the same spatial position from the perspective of $m_a$.

\paragraph{Semantic and Geometric Feature Extraction}
For a 2D mask generated by the VFM in frame $x_t$, its bounding box is cropped from $C_t$ at multiple scales and fed into CLIP~\cite{radford2021learning} visual encoder to produce the open-vocabulary semantic feature.

For geometric feature extraction, the Marching Cubes algorithm~\cite{lorensen1998marching} is first applied to $\mathit{Vol}_{t}$ to obtain the so-far reconstructed scene point cloud $S_t$. This point cloud is then processed by FCGF~\cite{choy2019fully} to generate per-point features. Finally, we identify the points that lie within the voxel set of the mask and aggregate their point-wise geometric features using average pooling to obtain the final geometric feature for the mask.


%-------------------------------------------------------------------------
\subsection{Online Mask Merging}
\label{subsec:online_mask_merging}
To obtain real-time 3D segmentation results and avoid the continuous increase in the number of detected masks, the online mask merging operation is applied to identify masks belonging to the same 3D instance and merge them into new masks. To fully leverage all available information up to the current timestamp $t$, our online merging strategy determines which masks should be merged based on the following criteria: (a) inclusion ratio, (b) semantic similarity, (c) geometric similarity, and (d) consensus from third-view perspectives. In the following context, we first introduce our zero-shot online merging strategy, followed by the associated updating operations for the Global Mask Database $G_t$.

\paragraph{Mask Merging Strategy}
In our setting, its not feasible to evaluate whether a pair of masks should be merged based on their spatial associations extracted from all views, as global observations are not available until the entire input sequence has been acquired. Therefore, more robust metrics are necessary to make informed decisions in real-time.

In general, we consider two masks to belong to the same 3D instance if either they are sufficiently similar overall, or there are enough third-view masks supporting their merging.

For the first criterion, we compute the overall similarity for all $n_t$ masks in $G_t$, incorporating their inclusion ratio, semantic similarity, and geometric similarity. The Overall Similarity Matrix $\mathit{Sim}_t \in \mathbb{R}^{n_t \times n_t}$ is computed using the following formula:
\begin{equation}
    \mathit{Sim}_t=\frac{1}{2}(\mathit{IR}_t + {\mathit{IR}_t}^{\top}) + F^S_t {F^S_t}^{\top} + F^G_t {F^G_t}^{\top}
    \label{eq:sim}
\end{equation}
where the first term represents the mutual inclusion ratio between masks, while the second and third terms denote their semantic and geometric similarities respectively.

Additionally, we import the concept of "view consensus", adapted from MaskClustering~\cite{yan2024maskclustering} with some modifications to better fit the online task. For any two masks $m_a$ and $m_b$, if there exist another mask $m_c$ that satisfies the following conditions: 
\begin{equation}
    ( ir_{(c,a)} > \tau_1 ) \cap ( ir_{(c,b)} > \tau_1 )
    \label{eq:including}
\end{equation}
where $\tau_1=0.8$ is a threshold for inclusion, and:
\begin{equation}
    ( ir_{(a,c)} > \tau_2 ) \cap ( ir_{(b,c)} > \tau_2 )
    \label{eq:included}
\end{equation}
where $\tau_2=0.1$ is a threshold for being included, then $m_c$ is considered as a \textbf{supporter} of $(m_a, m_b)$.

The condition in \cref{eq:including} indicates that from the perspective of $m_c$, both $m_a$ and $m_b$ are part of the same object, while the condition in \cref{eq:included} ensures that from both $m_a$ and $m_b$'s perspectives, $m_c$ is visible.

% \input{fig/fig_supporter_num_mat}
Notably, the supporter number matrix $A_t$, where the element at position $[a, b]$ denotes the supporter number of $(m_a,m_b)$, can be computed efficiently from $I_t$ and $W_t$ as follows:
\begin{equation}
\begin{aligned}
      B &= ({I_t}^{\top} > \tau_1) \& (\mathit{I}_t > \tau_2) \\
    A_t &= B W {B}^{\top}
    \label{eq:supporter_num_mat}
\end{aligned}
\end{equation}
where $B \in \mathbb{R}^{n_t \times n_t}$ is a binary matrix, and $\&$ denotes element-wise "and" operation between two matrices. 
% \cref{fig:supporter_num_mat} provides an example of this computing process.

Combing the above two criteria, whether a pair of masks $(m_a, m_b)$ needs to be merged is evaluated by the following condition:
\begin{equation}
    ( \mathit{Sim}_t[a,b] > \tau_{sim} ) \cup ( A_t[a,b] > \tau_{supporter} )
    \label{eq:merge}
\end{equation}
where $\tau_{sim}$ and $\tau_{supporter}$ are thresholds for overall similarity and supporter number respectively. 
% \cref{eq:merge} indicates that two masks should be merged if either they are sufficiently similar in different aspects, or if there are enough third-view masks supporting their merging.


\paragraph{Updating the Global Mask Database}
\label{subsubsec:merge_update}
\input{fig/fig_mapping_table}

After determining which masks need to be merged, the corresponding data structure in the Global Mask Database $G_t$ must be updated synchronously. All masks in $G_t$ can now be categorized into two groups: retained masks (those that do not need merging) and combined masks (those that will be merged with others to form a new mask). The merging and updating stage involves the following steps:

\begin{enumerate}
\item \textbf{Updating $\mathbf{V_t}$ and $\mathbf{W_t}$:} The corresponding voxel set of a new mask is formed by taking the union of the voxel sets of its constituent masks, and the weight of this new mask is the sum of their individual weights.

\item \textbf{Updating $\mathbf{F^G_t}$ and $\mathbf{F^S_t}$:} For each newly created mask, its semantic feature is aggregated from its constituent mask by average pooling, and its geometric feature is re-extracted using its updated voxel set from the latest reconstructed point cloud.

\item \textbf{Re-assigning global mask ID:} Each mask after merging, including both retained masks and new masks, is assigned a new global mask ID within the Global Mask Set. We maintain a mapping table that tracks the original ID of each mask and its corresponding current global mask ID, and only this table is updated accordingly. This approach eliminates the need for frequent updates of the hash table $H_t$, significantly reducing time consumption. An illustration of this process is given in \cref{fig:mapping_table}.

\item \textbf{Updating $\mathbf{I_t}$}: Since all masks are reorganized, their corresponding inclusion matrix should be synchronized. Specifically:
(1) the rows and columns corresponding to remained masks stay unchanged, while thoses for the combined masks are removed. 
(2) rows and columns for new masks are then appended, and each element are recalculated by querying $H_t$ with its updated voxel set.
\end{enumerate}


%-------------------------------------------------------------------------
\subsection{Implementation Details}
\label{subsec:imple_detail}
% To ensure the efficiency of our method, we segment input frames at fixed intervals of 10 frames, with a mask merging interval of 50 frames. At the end of input sequence, we apply the same post-processing approach as in OVIR-3D~\cite{lu2023ovir}, to refine detected 3D instances.  For the final 3D instance prediction, only merged masks with weights greater than $\tau_{weight}=5$ will be considered. For the hyperparameters, we set $\tau_{sim}=2.3, \tau_{supporter}=5$. We test our method on an NVIDIA RTX 4090 GPU.
To ensure the efficiency of our method, we select keyframes at fixed intervals of 10 frames, with segmentation applied only to these keyframes. The mask merging operation is performed every 5 keyframes. At the end of input sequence, we apply the same post-processing approach as in OVIR-3D~\cite{lu2023ovir}, to refine detected 3D instances.  For the final 3D instance prediction, only merged masks with weights greater than $\tau_{weight}=5$ will be considered as valid instances and reported. The hyperparameters are set as $\tau_{sim}=2.3, \tau_{supporter}=5$. We test our method on an NVIDIA RTX 4090 GPU.



==> table/tabel_intermediate_results.tex <==
\begin{table*}[h]

\centering
\setlength{\tabcolsep}{10pt}  % 增加列间距（默认是 6pt，可以根据需要调整）
\renewcommand{\arraystretch}{1.25}  % 增加行间距

\begin{tabular}{l|ccc|ccc|ccc}
\specialrule{2.0pt}{0pt}{0pt}  % 顶部粗线

\textbf{Method} & \multicolumn{3}{c|}{\textbf{25\%}} & \multicolumn{3}{c|}{\textbf{50\%}} & \multicolumn{3}{c}{\textbf{75\%}} \\

 & $AP$ & $AP_{50}$ & $AP_{25}$ & $AP$ & $AP_{50}$ & $AP_{25}$ & $AP$ & $AP_{50}$ & $AP_{25}$ \\
\specialrule{1.0pt}{0pt}{0pt}

EmbodiedSAM~\cite{xu2024embodiedsam} & 12.1 & 28.5 & 48.6 & 11.8 & 28.6 & 48.1 & 12.2 & 26.9 & 50.4 \\
Ours & \textbf{16.6} & \textbf{36.2} & \textbf{59.3} & \textbf{16.0} & \textbf{36.1} & \textbf{60.7} & \textbf{16.8} & \textbf{35.1} & \textbf{58.8} \\

\specialrule{2.0pt}{0pt}{0pt}  % 底部粗线
\end{tabular}

\caption{Intermediate segmentation results of online methods on SceneNN Dataset~\cite{hua2016scenenn}. }
\label{tab:inter_result}

\end{table*}

==> table/tabel_intermediate_results2.tex <==
\begin{table*}[h]

\centering
\setlength{\tabcolsep}{6pt}  % 增加列间距（默认是 6pt，可以根据需要调整）
\renewcommand{\arraystretch}{1.25}  % 增加行间距

\begin{tabular}{l|cc|ccc|ccc|ccc}
\specialrule{2.0pt}{0pt}{0pt}  % 顶部粗线

\textbf{Method} & \textbf{ Online} & \textbf{Zero-shot} & \multicolumn{3}{c|}{\textbf{25\%}} & \multicolumn{3}{c|}{\textbf{50\%}} & \multicolumn{3}{c}{\textbf{75\%}} \\

 & & & $AP$ & $AP_{50}$ & $AP_{25}$ & $AP$ & $AP_{50}$ & $AP_{25}$ & $AP$ & $AP_{50}$ & $AP_{25}$ \\
\specialrule{1.0pt}{0pt}{0pt}

EmbodiedSAM~\cite{xu2024embodiedsam} & \ding{51} & \ding{55} & 12.1 & 28.5 & 48.6 & 11.8 & 28.6 & 48.1 & 12.2 & 26.9 & 50.4 \\
Ours & \ding{51} & \ding{51} & \textbf{16.6} & \textbf{36.2} & \textbf{59.3} & \textbf{16.0} & \textbf{36.1} & \textbf{60.7} & \textbf{16.8} & \textbf{35.1} & \textbf{58.8} \\

\specialrule{2.0pt}{0pt}{0pt}  % 底部粗线
\end{tabular}

\caption{Intermediate segmentation results of online methods on SceneNN Dataset~\cite{hua2016scenenn}. }
\label{tab:inter_result}

\end{table*}

==> table/table_ablation_hyperparameter.tex <==
\begin{table}[h]

\centering
\setlength{\tabcolsep}{10pt}  % 增加列间距（默认是 6pt，可以根据需要调整）
\renewcommand{\arraystretch}{1.25}  % 增加行间距

\begin{tabular}{l|ccc}
\specialrule{1.0pt}{0pt}{0pt}  % 顶部粗线
  & $AP$ & $AP_{50}$ & $AP_{25}$ \\
\specialrule{1.0pt}{0pt}{0pt}

$\tau_1$ &  &  &  \\
$\tau_2$ &  &  &  \\
$\tau_{sim}$ &  &  &  \\
$\tau_{supporter}$ &  &  &  \\

\specialrule{1.0pt}{0pt}{0pt}  % 底部粗线
\end{tabular}

\caption{Ablation study on Hyperparameters. }
\label{tab:ablation_hyperparameter}

\end{table}

==> table/table_ablation_scene.tex <==
\begin{table}[h]

\centering
\small
\setlength{\tabcolsep}{5pt}  % 增加列间距（默认是 6pt，可以根据需要调整）
\renewcommand{\arraystretch}{1.25}  % 增加行间距

\begin{tabular}{l|ccc}
\specialrule{1.0pt}{0pt}{0pt}  % 顶部粗线
  & $AP$ & $AP_{50}$ & $AP_{25}$ \\
\specialrule{1.0pt}{0pt}{0pt}

VoxelHashing(voxel size=2.5cm) & \textbf{16.8} & \textbf{32.7} & \textbf{51.7} \\
VoxelHashing(voxel size=5cm) &  &  &  \\
Back-projected point cloud &  &  &  \\
3D GS point cloud &  &  &  \\


\specialrule{1.0pt}{0pt}{0pt}  % 底部粗线
\end{tabular}

\caption{Ablation study on different scene representation. }
\label{tab:ablation_scene}

\end{table}

==> table/table_example.tex <==
\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

==> table/table_rebuttal_SAM.tex <==
\begin{table}[h]
\captionsetup{aboveskip=0pt, belowskip=0pt} % 设置标题上下间距
\centering
\small
\vspace{-6pt}
\begin{tabular}{l|ccc}
\specialrule{1.0pt}{0pt}{0pt}  % 顶部粗线
  & $AP$ & $AP_{50}$ & $AP_{25}$ \\
\specialrule{0.5pt}{0pt}{0pt}

SAM3D$^*\dag$ & 9.3 & 22.5 & 47.9 \\
Ours(w.SAM) & \textbf{14.4} & \textbf{29.1} & \textbf{51.4} \\
% Ours & \textbf{16.8} & \textbf{32.7} & \textbf{51.7} \\

\specialrule{1.0pt}{0pt}{0pt}  % 底部粗线
\end{tabular}
\vspace{2pt}
% \caption{Ablation study on }
\label{tab:rebuttal_sam}

\end{table}

==> table/table_rebuttal_weight.tex <==
\begin{table}[h]
\captionsetup{aboveskip=0pt, belowskip=0pt} % 设置标题上下间距
\centering
\small

\begin{tabular}{l|cccccc}
\specialrule{1.0pt}{0pt}{0pt}  % 顶部粗线
$\tau_{\text{weight}}$  & 3 & 4 & 5 & 6 & 7 & 8 \\
\specialrule{0.5pt}{0pt}{0pt}

$AP_{25}$ & 50.2 & \textbf{51.7} & \textbf{51.7} & \textbf{51.7} & 51.2 & 50.6 \\
$AP_{50}$ & 29.5 & 32.7 & 32.7 & 32.7 & \textbf{32.9} & 30.8 \\
$AP$ & 16.1 & \textbf{16.8} & \textbf{16.8} & 16.5 & 16.2 & 15.8 \\

\specialrule{1.0pt}{0pt}{0pt}  % 底部粗线
\end{tabular}

\label{tab:rebuttal_mask_weight}

\end{table}

==> table/table_scannet200.tex <==
\begin{table*}[h]

\centering
\setlength{\tabcolsep}{12pt}  % 增加列间距（默认是 6pt，可以根据需要调整）

\begin{tabular}{lcccccc}
\specialrule{2.0pt}{0pt}{0pt}  % 顶部粗线
Method & Online & Zero-shot & $AP$ & $AP_{50}$ & $AP_{25}$ & Speed \\
\specialrule{1.0pt}{0pt}{0pt}
Mask3D~\cite{schult2022mask3d} & \ding{55} & \ding{55} & 39.7 & 53.6 & 62.5 & - \\
OpenMask3D~\cite{takmaz2023openmask3d} & \ding{55} & \ding{55} & 39.7 & 53.6 & 62.5 & - \\
EmbodiedSAM~\cite{xu2024embodiedsam} & \ding{51} & \ding{55} & 28.8 & 42.7 & 54.2 & 1 \\
OVIR-3D~\cite{lu2023ovir} & \ding{55} & \ding{51} & 14.4 & 27.5 & 38.8 & - \\
MaskClustering~\cite{yan2024maskclustering} & \ding{55} & \ding{51} & 19.7 & 36.4 & 51.4 & - \\
\hline
SAM3D~\cite{yang2023sam3d} & \ding{51} & \ding{51} & \textcolor{red}{17.8} & \textcolor{red}{30.6} & \textcolor{red}{48.5} & 1 \\
Ours & \ding{51} & \ding{51} & 18.6 & 36.1 & 53.5 & 1 \\
\specialrule{2.0pt}{0pt}{0pt}  % 底部粗线
\end{tabular}

\caption{Class-agnostic 3D instance segmentation results on ScanNet200}
\label{tab:scannet200}

\end{table*}

==> table/table_suppl_inter.tex <==
\begin{table*}[ht]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}  % 增加列间距（默认是 6pt，可以根据需要调整）
    \renewcommand{\arraystretch}{1.05}  % 增加行间距

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 子表 (a), 25% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{tabular}{c||ccc|ccc||ccc|ccc||ccc|ccc}
        \specialrule{1.0pt}{0pt}{0pt}  % 顶部粗线
        \multirow{3}*{\textbf{Scene}} & \multicolumn{6}{c||}{\textbf{25\%}} & \multicolumn{6}{c||}{\textbf{50\%}} & \multicolumn{6}{c}{\textbf{75\%}} \\
        \cline{2-19}  % 顶部粗线
        ~ & \multicolumn{3}{c|}{\textbf{EmbodiedSAM$^{**}$}} & \multicolumn{3}{c||}{\textbf{Ours$^*$}} & \multicolumn{3}{c|}{\textbf{EmbodiedSAM$^{**}$}} & \multicolumn{3}{c||}{\textbf{Ours$^*$}} & \multicolumn{3}{c|}{\textbf{EmbodiedSAM$^{**}$}} & \multicolumn{3}{c}{\textbf{Ours$^*$}} \\
        ~ & $AP$ & $AP_{50}$ & $AP_{25}$ & $AP$ & $AP_{50}$ & $AP_{25}$ & $AP$ & $AP_{50}$ & $AP_{25}$ & $AP$ & $AP_{50}$ & $AP_{25}$ & $AP$ & $AP_{50}$ & $AP_{25}$ & $AP$ & $AP_{50}$ & $AP_{25}$ \\
        \specialrule{1.0pt}{0pt}{0pt}
        005 & 7.1 & 17.5 & \textbf{51.0} & \textbf{7.9} & \textbf{25.6} & 47.2 & 8.5 & 17.4 & 42.3 & \textbf{11.9} & \textbf{34.0} & \textbf{60.2} & 9.3 & 20.2 & 53.5 & \textbf{14.2} & \textbf{36.9} & \textbf{58.6} \\
        011 & 11.5 & 25.7 & 42.9 & \textbf{31.8} & \textbf{51.3} & \textbf{61.3} & 15.8 & 35.1 & 55.2 & \textbf{29.4} & \textbf{59.8} & \textbf{68.2} & 17.8 & 33.3 & 59.1 & \textbf{33.9} & \textbf{63.6} & \textbf{70.1} \\
        015 & 14.7 & 34.1 & 47.3 & \textbf{38.2} & \textbf{60.1} & \textbf{81.2} & 17.2 & 37.9 & 38.1 & \textbf{27.9} & \textbf{40.2} & \textbf{52.5} & 12.8 & 27.1 & 41.3 & \textbf{23.9} & \textbf{34.6} & \textbf{45.7} \\
        030 & \textbf{12.2} & 20.9 & 37.4 & 8.5 & \textbf{25.1} & \textbf{48.4} & 14.3 & 22.7 & 40.1 & \textbf{15.7} & \textbf{29.3} & \textbf{48.5} & \textbf{18.3} & \textbf{30.6} & \textbf{47.9} & 14.6 & 24.4 & 41.8 \\
        054 & \textbf{14.3} & \textbf{45.0} & 64.3 & 11.9 & 35.9 & \textbf{65.8} & \textbf{19.7} & \textbf{60.6} & \textbf{76.3} & 18.7 & 42.0 & 69.5 & 16.2 & \textbf{41.1} & \textbf{67.5} & \textbf{17.8} & 39.3 & 61.7 \\
        080 & 7.8 & 13.0 & \textbf{52.4} & \textbf{20.2} & \textbf{48.0} & 49.3 & 5.1 & 16.5 & 35.6 & \textbf{16.3} & \textbf{39.7} & \textbf{57.2} & 3.1 & 7.2 & \textbf{33.9} & 13.0 & \textbf{30.1} & \textbf{51.2} \\
        089 & \textbf{6.6} & \textbf{23.8} & 40.4 & 3.6 & 9.5 & \textbf{44.9} & 4.8 & \textbf{18.9} & 41.0 & \textbf{5.6} & 16.5 & \textbf{49.0} & \textbf{5.0} & \textbf{19.0} & 45.5 & 4.7 & 17.9 & \textbf{52.7} \\
        093 & 17.8 & 46.6 & 63.2 & \textbf{29.8} & \textbf{50.0} & \textbf{72.9} & 16.7 & \textbf{39.9} & 59.7 & \textbf{19.3} & 37.7 & \textbf{63.3} & 13.6 & 31.0 & 58.8 & \textbf{18.2} & \textbf{33.9} & \textbf{63.0} \\
        096 & \textbf{11.7} & \textbf{36.8} & 38.3 & 9.5 & 18.7 & \textbf{59.5} & 10.0 & \textbf{35.3} & 42.8 & \textbf{14.0} & 25.8 & \textbf{61.2} & 11.5 & \textbf{41.5} & 49.0 & \textbf{12.7} & 24.8 & \textbf{66.0} \\
        243 & 11.1 & 22.9 & \textbf{62.5} & \textbf{17.1} & \textbf{45.5} & 59.7 & 9.1 & 20.2 & \textbf{63.8} & \textbf{10.0} & \textbf{31.1} & 60.8 & 11.7 & 23.1 & \textbf{66.7} & \textbf{14.8} & \textbf{39.6} & \textbf{66.7} \\
        263 & 26.5 & 52.2 & 61.5 & \textbf{39.0} & \textbf{71.6} & \textbf{86.8} & 29.4 & 52.2 & 69.2 & \textbf{35.4} & \textbf{66.8} & \textbf{76.9} & 22.4 & 39.2 & 57.1 & \textbf{32.3} & \textbf{60.8} & \textbf{74.2} \\
        322 & 9.3 & 22.2 & 35.0 & \textbf{16.7} & \textbf{35.9} & \textbf{61.1} & 11.2 & 24.7 & 37.5 & \textbf{15.5} & \textbf{41.9} & \textbf{74.3} & 18.3 & 38.0 & 47.2 & \textbf{24.1} & \textbf{48.7} & \textbf{77.3} \\
        \specialrule{1.0pt}{0pt}{0pt}  % 底部粗线
    \end{tabular}



\caption{\textbf{Intermediate instance segmentation results at different sequence completion on SceneNN~\cite{hua2016scenenn}.} The instance segmentation results are evaluated by mapping from the reconstructed point cloud or mesh to ground truth point cloud through point correspondences. $^*$: Zero-shot method, $^{**}$: Learning-based method.}
\label{tab:supp_inter_result}
\end{table*}


